CR3DT: Camera-RADAR Fusion for 3D Detection and Tracking

To enable self-driving vehicles accurate detection and tracking of surrounding objects is essential. While Light Detection and Ranging (LiDAR) sensors have set the benchmark for high-performance systems, the appeal of camera-only solutions lies in their cost-effectiveness. Notably, despite the prevalent use of Radio Detection and Ranging (RADAR) sensors in automotive systems, their potential in 3D detection and tracking has been largely disregarded due to data sparsity and measurement noise. As a recent development, the combination of RADARs and cameras is emerging as a promising solution. This paper presents Camera-RADAR 3D Detection and Tracking (CR3DT), a camera-RADAR fusion model for 3D object detection, and Multi-Object Tracking (MOT). Building upon the foundations of the State-of-the-Art (SotA) camera-only BEVDet architecture, CR3DT demonstrates substantial improvements in both detection and tracking capabilities, by incorporating the spatial and velocity information of the RADAR sensor. Experimental results demonstrate an absolute improvement in detection performance of 5.3% in mean Average Precision (mAP) and a 14.9% increase in Average Multi-Object Tracking Accuracy (AMOTA) on the nuScenes dataset when leveraging both modalities. CR3DT bridges the gap between high-performance and cost-effective perception systems in autonomous driving, by capitalizing on the ubiquitous presence of RADAR in automotive applications. The code is available at: https://github.com/ETH-PBL/CR3DT.

==> src/det_abl_slim.tex <==
\begin{table}[ht]
    \begin{subtable}{.98\columnwidth}
        \centering
        \begin{tabular}{l|c|c}
            \toprule
            \#  & \textbf{\gls{map} [\%]$\uparrow$} & \textbf{\acrshort{mave}[$\frac{m}{s}$]$\downarrow$} \\
            \midrule
            % ablation 1: https://wandb.ai/ferrari-bandits/BEVDet/runs/ghwcpve5
            1 & \textbf{34.66} & \textbf{0.45}  \\
            % ablation 2: https://wandb.ai/ferrari-bandits/BEVDet/runs/is3yv1nk
            10 & 32.06  & 0.52  \\
            \bottomrule
        \end{tabular}
        \caption{$z$-dimension discretization}
        \label{tab:ablation_zdim}
    \end{subtable}%
    \hfill
    \begin{subtable}{.98\columnwidth}
        \centering
        \begin{tabular}{l|c|c}
            \toprule
            % ablation 3 is with late fusion: https://wandb.ai/ferrari-bandits/BEVDet/runs/8lusbxdp
            \textbf{LF} & \textbf{\gls{map} [\%]$\uparrow$} & \textbf{\acrshort{mave}[$\frac{m}{s}$]$\downarrow$} \\
            \midrule
            Yes & \textbf{35.15} & 0.47  \\
            % ablation 4 is ablation 2: https://wandb.ai/ferrari-bandits/BEVDet/runs/is3yv1nk
            No & 34.66 & \textbf{0.45}  \\
            \bottomrule
        \end{tabular}
        \caption{Late Fusion for Radar}
        \label{tab:ablation_latefus}
    \end{subtable}
    \caption{Architecture ablation experiments}
    \label{tab:ablation}
\end{table}

==> src/maintab_full.tex <==
\begin{table*}[t]
\centering
\caption{Tracking results on the \emph{nuScenes} validation set, featuring only detection models in the \emph{restricted model class}. The baseline is represented by the vanilla \emph{BEVDet} model \cite{bevdet, wang2023streampetr}. Tracking was performed on perspective image embeddings following \cite{cc3dt, qdtrack}. \emph{C, R} denote the sensor modalities, camera, and \gls{radar} respectively. Computational measurements were performed on a GeForce RTX 3090.}
\resizebox{\textwidth}{!}{%
\begin{tabular}{l|c|c|c|c|c|ccc|ccc}
\toprule
\textbf{Tracking Models} & \textbf{Input} & \textbf{thresh} & \textbf{weight} & \textbf{sim} & \textbf{Latency [ms] $\downarrow$} & \multicolumn{3}{|c|}{\textbf{Detection Performance}} & \multicolumn{3}{|c}{\textbf{Tracking Performance}} \\
\midrule
& & & & & & \textbf{\gls{map} [\%]$\uparrow$} & \textbf{\gls{nds} [\%]$\uparrow$} & \textbf{\acrshort{mave} [$\frac{m}{s}$]$\downarrow$} & \textbf{\gls{amota} [\%]$\uparrow$} & \textbf{\gls{amotp} [m]$\downarrow$} & \textbf{\gls{nds} [\#] $\downarrow$}\\
\midrule
BEVDet + CC-3DT & C &  & & & \textbf{88.1} & 30.05 & 36.52 & 0.92 & 22.4 & 1.476 & ass\\ %Baseline
% baseline wandb: https://wandb.ai/ferrari-bandits/BEVDet/runs/n14i4gso
% and NUSC json: 
% BUT ACTUALLY, a better baseline (on all metrics) is here
% https://wandb.ai/ferrari-bandits/BEVDet/runs/j2fhtfzc
% But anyway, they all overperform the orignal BEVDET so idk if we should
\midrule[0.5\lightrulewidth]
BEVDet + CC-3DT & C  & & & & \textbf{88.1} & 30.05 & 36.52 & 0.92 & 22.4 & 1.476 & ass\\ %Baseline
\midrule

\acrshort{cr3d} + CC-3DT   & C+R & def & def & cos & 90.04 & \textbf{35.15 (+5.10)} & \textbf{45.61 (+9.09)} & \textbf{0.47 (-0.45)} &  \todo[]{  new data} & \todo[]{  new data} & ass \\ %cr3dt and cc3dt 
\midrule[0.5\lightrulewidth]

\acrshort{cr3d} + CC-3DT   & C+R & 0.30 & def & cos & 90.04 & \textbf{35.15 (+5.10)} & \textbf{45.61 (+9.09)} & \textbf{0.47 (-0.45)} &  \todo[]{  new data} & \todo[]{  new data} & ass \\ %cr3dt and cc3dt 
\midrule[0.5\lightrulewidth]

\acrshort{cr3d} + CC-3DT   & C+R & def & 75-25 & cos & 90.04 & \textbf{35.15 (+5.10)} & \textbf{45.61 (+9.09)} & \textbf{0.47 (-0.45)} &  \todo[]{  new data} & \todo[]{  new data} & ass \\ %cr3dt and cc3dt 
\midrule[0.5\lightrulewidth]

\acrshort{cr3d} + CC-3DT & C+R & 0.30 & 75-25 & cos & 90.04 & \textbf{35.15 (+5.10)} & \textbf{45.61 (+9.09)} & \textbf{0.47 (-0.45)} &  \todo[]{  new data} & \todo[]{  new data} & ass \\ %cr3dt and cc3dt 
\midrule[0.5\lightrulewidth]

\acrshort{cr3d} + CC-3DT++ & C+R  & 0.30 & 75-25 & vel & 90.04 & \textbf{35.15 (+5.10)} & \textbf{45.61 (+9.09)} & \textbf{0.47 (-0.45)} &  \todo[]{  new data} & \todo[]{  new data} & ass \\ %cr3dt and cc3dt only image embeddings
\bottomrule
\end{tabular}%
}
\label{tab:tracking}
\end{table*}


==> src/maintab_fullv2.tex <==

\begin{table*}[t]
\centering
\caption{Tracking results on the \emph{nuScenes} validation set, featuring only detection models in the \emph{restricted model class}. The baseline is represented by the vanilla \emph{BEVDet} model \cite{bevdet, wang2023streampetr}. Tracking was performed on perspective image embeddings following \cite{cc3dt, qdtrack}. \emph{C, R} denote the sensor modalities, camera, and \gls{radar} respectively. Computational measurements were performed on a GeForce RTX 3090.}
\resizebox{\textwidth}{!}{%
\begin{tabular}{l|c|c|c|c|c|ccc|ccc}
\toprule
\textbf{Tracking Models} & \textbf{Input} & \textbf{thresh} & \textbf{weight} & \textbf{velsim} & \textbf{Latency [ms] $\downarrow$} & \multicolumn{3}{|c|}{\textbf{Detection Performance}} & \multicolumn{3}{|c}{\textbf{Tracking Performance}} \\
\midrule
& & & & & & \textbf{\gls{map} [\%]$\uparrow$} & \textbf{\gls{nds} [\%]$\uparrow$} & \textbf{\acrshort{mave} [$\frac{m}{s}$]$\downarrow$} & \textbf{\gls{amota} [\%]$\uparrow$} & \textbf{\gls{amotp} [m]$\downarrow$} & \textbf{\gls{nds} [\#] $\downarrow$}\\
\midrule
BEVDet + CC-3DT & C &  & & & \textbf{88.1} & 30.05 & 36.52 & 0.92 & 22.4 & 1.476 & ass\\ %Baseline
% baseline wandb: https://wandb.ai/ferrari-bandits/BEVDet/runs/n14i4gso
% and NUSC json: 
% BUT ACTUALLY, a better baseline (on all metrics) is here
% https://wandb.ai/ferrari-bandits/BEVDet/runs/j2fhtfzc
% But anyway, they all overperform the orignal BEVDET so idk if we should
\midrule[0.5\lightrulewidth]
BEVDet + CC-3DT & C  & & & & \textbf{88.1} & 30.05 & 36.52 & 0.92 & 22.4 & 1.476 & ass\\ %Baseline
\midrule

\acrshort{cr3d} + CC-3DT   & C+R & \xmark & \xmark & \xmark & 90.04 & \textbf{35.15 (+5.10)} & \textbf{45.61 (+9.09)} & \textbf{0.47 (-0.45)} &  \todo[]{  new data} & \todo[]{  new data} & ass \\ %cr3dt and cc3dt 
\midrule[0.5\lightrulewidth]

\acrshort{cr3d} + CC-3DT   & C+R & \cmark & \xmark & \xmark & 90.04 & \textbf{35.15 (+5.10)} & \textbf{45.61 (+9.09)} & \textbf{0.47 (-0.45)} &  \todo[]{  new data} & \todo[]{  new data} & ass \\ %cr3dt and cc3dt 
\midrule[0.5\lightrulewidth]

\acrshort{cr3d} + CC-3DT   & C+R & \xmark & \cmark & \xmark & 90.04 & \textbf{35.15 (+5.10)} & \textbf{45.61 (+9.09)} & \textbf{0.47 (-0.45)} &  \todo[]{  new data} & \todo[]{  new data} & ass \\ %cr3dt and cc3dt 
\midrule[0.5\lightrulewidth]

\acrshort{cr3d} + CC-3DT & C+R & \cmark & \cmark & \xmark & 90.04 & \textbf{35.15 (+5.10)} & \textbf{45.61 (+9.09)} & \textbf{0.47 (-0.45)} &  \todo[]{  new data} & \todo[]{  new data} & ass \\ %cr3dt and cc3dt 
\midrule[0.5\lightrulewidth]

\acrshort{cr3d} + CC-3DT++ & C+R  & \cmark & \cmark & \cmark & 90.04 & \textbf{35.15 (+5.10)} & \textbf{45.61 (+9.09)} & \textbf{0.47 (-0.45)} &  \todo[]{  new data} & \todo[]{  new data} & ass \\ %cr3dt and cc3dt only image embeddings
\bottomrule
\end{tabular}%
}
\label{tab:tracking}
\end{table*}


==> src/maintab_sep.tex <==
\begin{table*}[t]
\centering
\caption{Tracking results on the \emph{nuScenes} validation set, featuring only detection models in the \emph{restricted model class}. The baseline is represented by the vanilla \emph{BEVDet} model \cite{bevdet, wang2023streampetr}. Tracking was performed on perspective image embeddings following \cite{cc3dt, qdtrack}. \emph{C, R} denote the sensor modalities, camera, and \gls{radar} respectively. Computational measurements were performed on a GeForce RTX 3090.}
\resizebox{\textwidth}{!}{%
\begin{tabular}{l|c|c|ccc|ccc}
\toprule
\textbf{Tracking Models} & \textbf{Input} & \textbf{Latency [ms] $\downarrow$} & \multicolumn{3}{|c|}{\textbf{Detection Performance}} & \multicolumn{3}{|c}{\textbf{Tracking Performance}} \\
\midrule
& & & \textbf{\gls{map} [\%]$\uparrow$} & \textbf{\gls{nds} [\%]$\uparrow$} & \textbf{\acrshort{mave} [$\frac{m}{s}$]$\downarrow$} & \textbf{\gls{amota} [\%]$\uparrow$} & \textbf{\gls{amotp} [m]$\downarrow$} & \textbf{\gls{nds} [\#] $\downarrow$}\\
\midrule
BEVDet + CC-3DT & C & \textbf{88.1} & 30.05 & 36.52 & 0.92 & 22.4 & 1.476 & ass\\ %Baseline
% baseline wandb: https://wandb.ai/ferrari-bandits/BEVDet/runs/n14i4gso
% and NUSC json: 
% BUT ACTUALLY, a better baseline (on all metrics) is here
% https://wandb.ai/ferrari-bandits/BEVDet/runs/j2fhtfzc
% But anyway, they all overperform the orignal BEVDET so idk if we should
\midrule[0.5\lightrulewidth]
BEVDet + CC-3DT++ & C & \textbf{88.1} & 30.05 & 36.52 & 0.92 & 22.4 & 1.476 & ass\\ %Baseline
\midrule
\acrshort{cr3d} + CC-3DT  & C+R & 90.04 & \textbf{35.15 (+5.10)} & \textbf{45.61 (+9.09)} & \textbf{0.47 (-0.45)} &  \todo[]{  new data} & \todo[]{  new data} & ass \\ %cr3dt and cc3dt 
% wandb: https://wandb.ai/ferrari-bandits/BEVDet/runs/8lusbxdp
\midrule[0.5\lightrulewidth]
\acrshort{cr3d} + CC-3DT++ & C+R & 90.04 & \textbf{35.15 (+5.10)} & \textbf{45.61 (+9.09)} & \textbf{0.47 (-0.45)} &  \todo[]{  new data} & \todo[]{  new data} & ass \\ %cr3dt and cc3dt only image embeddings
\bottomrule
\end{tabular}%
}
\label{tab:tracking}
\end{table*}


\begin{table*}[ht]
\resizebox{\textwidth}{!}{%
    \begin{subtable}{0.32\textwidth}
        \centering
        \begin{tabular}{l|c|c|c}
            \toprule
            \#  & \textbf{\gls{amota} [\%]$\uparrow$} & \textbf{\acrshort{ids}$\downarrow$} \\
            \midrule
            default(xx) & 0.xx & \textbf{0.45}  \\
            0.30 & 32.06  & 0.52  \\
            0.18 & 32.06  & 0.52  \\
            \bottomrule
        \end{tabular}
        \caption{Threshold ablation}
        \label{tab:ablation_zdim}
    \end{subtable}%
    \hfill
    \begin{subtable}{0.32\textwidth}
        \centering
        \begin{tabular}{l|c|c|c}
            \toprule
            \#  & \textbf{\gls{amota} [\%]$\uparrow$} & \textbf{\acrshort{ids}$\downarrow$} \\
            \midrule
            default(50-50?) & 0.xx & \textbf{0.45}  \\
            25-75 & 32.06  & 0.52  \\
            75-25 & 32.06  & 0.52  \\
            80-20 & 32.06  & 0.52  \\
            70-30 & 32.06  & 0.52  \\
            \bottomrule
        \end{tabular}
        \caption{Weighting ablation}
        \label{tab:ablation_latefus}
    \end{subtable}
    \hfill
    \begin{subtable}{0.32\textwidth}
        \centering
        \begin{tabular}{l|c|c}
            \toprule
            % ablation 3 is with late fusion: https://wandb.ai/ferrari-bandits/BEVDet/runs/8lusbxdp
            \textbf{velsim} & \textbf{\gls{map} [\%]$\uparrow$} & \textbf{\acrshort{mave}[$\frac{m}{s}$]$\downarrow$} \\
            \midrule
            cos sim (?) & \textbf{35.15} & 0.47  \\
            % ablation 4 is ablation 2: https://wandb.ai/ferrari-bandits/BEVDet/runs/is3yv1nk
            vel sim & 34.66 & \textbf{0.45}  \\
            \bottomrule
        \end{tabular}
        \caption{Velsim Ablation}
        \label{tab:ablation_latefus}
    \end{subtable}
    }
    \caption{Tracker Ablation experiments}
    \label{tab:ablation}
\end{table*}

==> src/maintab_sepv2.tex <==
\begin{table*}[t]
    \centering
    \caption{Tracking results on the \emph{nuScenes} validation set, featuring only detection models in the \emph{restricted model class}. The baseline is represented by the vanilla \emph{BEVDet} model \cite{bevdet, wang2023streampetr}. Tracking was performed on perspective image embeddings following \cite{cc3dt, qdtrack}. \emph{C, R} denote the sensor modalities, camera, and \gls{radar} respectively. Computational measurements were performed on a GeForce RTX 3090.}
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{l|c|c|ccc|ccc}
    \toprule
    \textbf{Tracking Models} & \textbf{Input} & \textbf{Latency [ms] $\downarrow$} & \multicolumn{3}{|c|}{\textbf{Detection Performance}} & \multicolumn{3}{|c}{\textbf{Tracking Performance}} \\
    \midrule
    & & & \textbf{\gls{map} [\%]$\uparrow$} & \textbf{\gls{nds} [\%]$\uparrow$} & \textbf{\acrshort{mave} [$\frac{m}{s}$]$\downarrow$} & \textbf{\gls{amota} [\%]$\uparrow$} & \textbf{\gls{amotp} [m]$\downarrow$} & \textbf{\gls{nds} [\#] $\downarrow$}\\
    \midrule
    BEVDet + CC-3DT & C & \textbf{88.1} & 30.05 & 36.52 & 0.92 & 22.4 & 1.476 & ass\\ %Baseline
    % baseline wandb: https://wandb.ai/ferrari-bandits/BEVDet/runs/n14i4gso
    % and NUSC json: 
    % BUT ACTUALLY, a better baseline (on all metrics) is here
    % https://wandb.ai/ferrari-bandits/BEVDet/runs/j2fhtfzc
    % But anyway, they all overperform the orignal BEVDET so idk if we should
    \midrule[0.5\lightrulewidth]
    BEVDet + CC-3DT++ & C & \textbf{88.1} & 30.05 & 36.52 & 0.92 & 22.4 & 1.476 & ass\\ %Baseline
    \midrule
    \acrshort{cr3d} + CC-3DT  & C+R & 90.04 & \textbf{35.15 (+5.10)} & \textbf{45.61 (+9.09)} & \textbf{0.47 (-0.45)} &  \todo[]{  new data} & \todo[]{  new data} & ass \\ %cr3dt and cc3dt 
    % wandb: https://wandb.ai/ferrari-bandits/BEVDet/runs/8lusbxdp
    \midrule[0.5\lightrulewidth]
    \acrshort{cr3d} + CC-3DT++ & C+R & 90.04 & \textbf{35.15 (+5.10)} & \textbf{45.61 (+9.09)} & \textbf{0.47 (-0.45)} &  \todo[]{  new data} & \todo[]{  new data} & ass \\ %cr3dt and cc3dt only image embeddings
    \bottomrule
    \end{tabular}%
    }
    \label{tab:tracking}
    \end{table*}
    
    \begin{table*}[ht]
        \resizebox{\textwidth}{!}{%
            \begin{subtable}{0.32\textwidth}
                \centering
                \begin{tabular}{l|cc|cc}
                    \toprule
                      & \multicolumn{2}{|c|}{\textbf{BEVDET bb}} & \multicolumn{2}{|c}{\textbf{CR3D bb}} \\
                    \midrule
                    \#  & \textbf{\gls{amota} \newline [\%]$\uparrow$} & \textbf{\acrshort{ids}$\downarrow$} & \textbf{\gls{amota} \newline [\%]$\uparrow$} & \textbf{\acrshort{ids}$\downarrow$} \\
                    \midrule
                    default(xx) & 0.xx & \textbf{0.45}  \\
                    0.30 & 32.06  & 0.52 & 32.06  & 0.52  \\
                    0.18 & 32.06  & 0.52 & 32.06  & 0.52  \\
                    \bottomrule
                \end{tabular}
                \caption{Threshold ablation}
                \label{tab:ablation_zdim}
            \end{subtable}%
            \hfill
            \begin{subtable}{0.32\textwidth}
                \centering
                \begin{tabular}{l|cc|cc}
                    \toprule
                      & \multicolumn{2}{|c|}{\textbf{BEVDET bb}} & \multicolumn{2}{|c}{\textbf{CR3D bb}} \\
                    \midrule
                    \#  & \textbf{\gls{amota} [\%]$\uparrow$} & \textbf{\acrshort{ids}$\downarrow$} & \textbf{\gls{amota} [\%]$\uparrow$} & \textbf{\acrshort{ids}$\downarrow$} \\
                    \midrule
                    default(50-50?) & 0.xx & \textbf{0.45}  \\
                    25-75      & 32.06  & 0.52 & 32.06  & 0.52  \\
                    75-25      & 32.06  & 0.52 & 32.06  & 0.52  \\
                    80-20      & 32.06  & 0.52 & 32.06  & 0.52  \\
                    70-30      & 32.06  & 0.52 & 32.06  & 0.52  \\
                    \bottomrule
                \end{tabular}
                \caption{Weighting ablation}
                \label{tab:ablation_latefus}
            \end{subtable}
            \hfill
            \begin{subtable}{0.32\textwidth}
                \centering
                \begin{tabular}{l|cc|cc}
                    \toprule
                      & \multicolumn{2}{|c|}{\textbf{BEVDET bb}} & \multicolumn{2}{|c}{\textbf{CR3D bb}} \\
                    \midrule
                    \#  & \textbf{\gls{amota} [\%]$\uparrow$} & \textbf{\acrshort{ids}$\downarrow$} & \textbf{\gls{amota} [\%]$\uparrow$} & \textbf{\acrshort{ids}$\downarrow$} \\
                    \midrule
                    cos sim & 32.06  & 0.52 & 32.06  & 0.52  \\
                    vel sim & 32.06  & 0.52 & 32.06  & 0.52  \\
                    \bottomrule
                \end{tabular}
                \caption{Velsim Ablation}
                \label{tab:ablation_latefus}
            \end{subtable}
            }
            \caption{Tracker Ablation experiments}
            \label{tab:ablation}
        \end{table*}
